A Unified Neural Coherence Model

Recently, neural approaches to coherence modeling have achieved state-of-the-art results in several evaluation tasks. However, we show that most of these models often fail on harder tasks with more realistic application scenarios. In particular, the existing models underperform on tasks that require the model to be sensitive to local contexts such as candidate ranking in conversational dialogue and in machine translation. In this paper, we propose a unified coherence model that incorporates sentence grammar, inter-sentence coherence relations, and global coherence patterns into a common neural framework. With extensive experiments on local and global discrimination tasks, we demonstrate that our proposed model outperforms existing models by a good margin, and establish a new state-of-the-art.

==> background.tex <==
\section{Background}
In this section, we introduce background knowledge of the proposed model for immediate reference. The proposed model is designed to capture local and global coherence in a text for better Thus, we first explain local and global coherence of text. Subsequently we introduce the siamese network \cite{Bromley93} and adaptive pairwise ranking loss. Finally, 

\subsection{Global vs. Local Coherence}
In general, the coherence models can be divided into local coherence and global coherence models by proximity of information, even though their underlying properties are closely connected \cite{Barzilay05,McKoon92}. Under the local coherence paradigm, the coherence of text is evaluated by capturing relations between sentences within a piece of the text \cite{McKoon92}. In contrast, the global coherence model evaluates a coherence by linking the globally separated textual information through a causal chain or network \cite{McKoon92}. Local and global coherence have been played central role in but

\subsection{Siamese Network}
The proposed model adopts a siamese architecture \cite{Bromley93} to learn and evaluate coherence in text. The siamese architecture consists of two sub-networks that share a set of parameters which take one input, respectively. The siamese is trained to find optimal network parameter $W$ that minimize the similarity metric $\mathcal{L}$ if the inputs are from the same class distribution, otherwise maximize it. 

% In coherence modeling case, two documents are fed into the siamese architecture and 
% The siamese architecture is used to learn a semantic distance of an input space by approximating it in a target space. More specifically, t
% Siamese network was first introduced by Bromley and LeCun for a handwritten signature verification . 

\subsection{Adaptive Pairwise Ranking Loss}
Coherence is relative so ranking loss is preferred \cite{Lin:2011}
We found out that the naive pairwise ranking loss unfairly penalize the locally positive sentences during learning

\subsection{Lightweight Convolution}




